The DESI Experiment Part I: Science,Targeting, and Survey Design

DESI (Dark Energy Spectroscopic Instrument) is a Stage IV ground-based dark energy experiment that will study baryon acoustic oscillations (BAO) and the growth of structure through redshift-space distortions with a wide-area galaxy and quasar redshift survey. To trace the underlying dark matter distribution, spectroscopic targets will be selected in four classes from imaging data. We will measure luminous red galaxies up to $z=1.0$. To probe the Universe out to even higher redshift, DESI will target bright [O II] emission line galaxies up to $z=1.7$. Quasars will be targeted both as direct tracers of the underlying dark matter distribution and, at higher redshifts ($ 2.1 < z < 3.5$), for the Ly-$\alpha$ forest absorption features in their spectra, which will be used to trace the distribution of neutral hydrogen. When moonlight prevents efficient observations of the faint targets of the baseline survey, DESI will conduct a magnitude-limited Bright Galaxy Survey comprising approximately 10 million galaxies with a median $z\approx 0.2$. In total, more than 30 million galaxy and quasar redshifts will be obtained to measure the BAO feature and determine the matter power spectrum, including redshift space distortions.

==> 2_Science/FoMtrades.tex <==
% This is an automatically generated file - don't edit (talk to Pat). 
0\% & 0\% & 0\% & 0\% & -- & 0\% & 37 & 22\% \\ 
50\% & 50\% & 50\% & 50\% & 14K & 50\% & 119 & 70\% \\ 
64\% & 64\% & 64\% & 64\% & 14K & 64\% & 136 & 80\% \\ 
100\% & 100\% & 100\% & 100\% & 14K & 100\% & 169 & 100\% \\ 
150\% & 150\% & 150\% & 150\% & 14K & 150\% & 202 & 119\% \\ 
\hline 
50\% & 50\% & 50\% & 50\% & 9K & 32\% & 85 & 50\% \\ 
100\% & 100\% & 100\% & 100\% & 9K & 64\% & 121 & 71\% \\ 
150\% & 150\% & 150\% & 150\% & 9K & 96\% & 145 & 86\% \\ 
\hline 
0\% & 100\% & 100\% & 100\% & 14K & 80\% & 158 & 93\% \\ 
50\% & 100\% & 100\% & 100\% & 14K & 90\% & 166 & 98\% \\ 
150\% & 100\% & 100\% & 100\% & 14K & 110\% & 172 & 101\% \\ 
\hline 
100\% & 0\% & 100\% & 100\% & 14K & 35\% & 132 & 78\% \\ 
100\% & 50\% & 100\% & 100\% & 14K & 67\% & 155 & 91\% \\ 
100\% & 150\% & 100\% & 100\% & 14K & 133\% & 180 & 106\% \\ 
\hline 
100\% & 100\% & 0\% & 100\% & 14K & 91\% & 133 & 79\% \\ 
100\% & 100\% & 50\% & 100\% & 14K & 96\% & 147 & 87\% \\ 
100\% & 100\% & 150\% & 100\% & 14K & 104\% & 188 & 111\% \\ 
100\% & 100\% & 3 visits & 100\% & 14K & 98\% & 168 & 99\% \\ 
100\% & 50\% & 3 visits & 100\% & 14K & 66\% & 153 & 90\% \\ 
\hline 
100\% & 100\% & 100\% & 0\% & 14K & 94\% & 163 & 96\% \\ 
100\% & 100\% & 100\% & 50\% & 14K & 97\% & 166 & 98\% \\ 
100\% & 100\% & 100\% & 150\% & 14K & 103\% & 173 & 102\% \\ 


==> 2_Science/science_bao_gal_reconstruction.tex <==
{\it Nikhil Padmanabhan}

Discuss galaxy reconstruction


==> 2_Science/science_bao_gal_systematics.tex <==
{\it Shirley Ho}

Discuss systematics relevant to galaxy BAO


==> 2_Science/science_bright.tex <==
\label{sec:bright}
\subsubsection{Overview}

\todo{Most of this moves to the target selection chapter.  There should be
some overview in 2.1 and maybe the exec summary.}

Roughly one week out of each month is not usable by the DESI Key
Project due to high background from scattered moonlight.  Here we
present a program with brighter galaxies and stars that could operate
in this bright time.  The bright-time program does not drive any
requirements on the DESI construction project and is not required to
meet the CD-0 Mission Need.  Therefore, we have not included it
elsewhere in this conceptual design report or the science requirements
document, save as separate points in Figures \ref{fig:binnedR} and \ref{fig:testGR}.  
For example, it is not included in the science discussion
and figures of merit presented earlier in this chapter.  

However, we argue in this subsection that this bright-time program can
produce compelling cosmological science, reinforcing and extending the
DESI Key Project goals.  The program can be executed with a modest
marginal increase in the operations budget.  By combining the program
into the same Science Collaboration as the Key Project, we will
maximize the benefits to both programs through broader expertise and
commonality of approach in both data reduction and science analysis.

What follows is the description of an initial design for a bright-time
program, developed by the DESI Collaboration Bright Time Committee.
Further simulation of the spectroscopic depth and tiling geometry is
needed to optimize the design, but the science reach is apparent.

After accounting for three nights per month of engineering time and
weather loss, we expect to have about 500 hours per year of good
observing conditions unused by the Key Project.  Assuming an observing
strategy with 6 configurations per hour (8-9 minutes plus overheads)
and five years of operations, this is 15,000 configurations.

Limiting the survey to declination north of --25$^\circ$ and Galactic
extinction $A_V<0.5$ mag allows a survey area of 20,000 square
degrees, about half of the sky.  We are considering footprints between
14,000 and 20,000 square degrees.  We expect to use a tiling density
similar to that of the Key Project, so that a typical point on the sky
is covered five times.  

Galaxies have surface brightnesses that are low enough as to be
substantially impacted by the increased background of bright time.
Nevertheless, our estimates are that DESI will be able to obtain
redshifts of galaxies as faint as $r=19.5$ in bright time in exposure
times around 20-30 minutes.  We expect substantial variation in this
number because bright-time conditions have a wide range of background
levels and because galaxies differ in their central surface brightness
and strength of emission lines.  Some galaxies will take only a single
exposure; others will take several.  We plan to do a rolling
acceptance of redshift success after each exposure, allowing 
fibers to target other nearby objects in future visits.

There are about 650 galaxies brighter than $r=19.5$ per square degree
at high Galactic latitude, dropping to 400 when viewed through 0.5 mag
of V-band Galactic extinction at lower Galactic latitude.  This is
reasonably matched to the DESI fiber density.  The majority of
galaxies at these magnitudes are low redshift systems (redshifts
between 0.1 to 0.4).  Low-redshift galaxies are substantially
clustered, and thus obtaining a high level of completeness will require
multiple visits.  Some fibers will be unable to reach a
viable galaxy target even on the first pass, and this fraction increases
on subsequent passes.  Bright stars are the natural secondary target,
and we expect that any bright galaxy survey with the DESI fiber
positioner will produce a very large sample of stars as a by-product.
This sample is also of high science interest, which we will describe
briefly below.

In summary, we anticipate a survey of about 10 million galaxies over
at least 14,000 and perhaps 20,000 square degrees, with a median redshift of 0.2 and extensive
coverage out to redshift 0.4.  Such a survey is a large step forward
with tremendous science reach.  Compared to the SDSS Main Galaxy
Sample, it is over twice the area and 15 times more galaxies.  It
would cover up to twice the volume of the BOSS LOWZ sample, but with much
higher sampling density.  It would include 100 times more galaxies
than the existing 6dF Galaxy Survey
\footnote{http://oldweb.aao.gov.au/local/www/6df/} and over 20 times
more than the planned TAIPAN survey, both of which cover most of the
southern hemisphere.  In depth, it is comparable to the GAMA survey
\footnote{http://www.gama-survey.org}, but with 50-fold more objects.
Roughly 1800 square degrees will overlap the DES survey region, and
up to 6000 square degrees will overlap the LSST $\delta<0$ primary
survey region.

\subsubsection{Cosmological Science in Bright Time}

\todo{This should move back into the previous sections.  Admittedly,
this will take a litte rewriting.  This first par might go to 2.1.}

The bright galaxy survey (BGS) differs from the DESI Key
Project in three important ways.  First, it is at low redshift,
when dark energy is dynamically more important.  Second, it will
produce a map with a much higher number density of tracers.  Third,
it will map the same volume with many different types of galaxies.
These differences lead to numerous cosmological opportunities.

\begin{enumerate}
\item The BGS will significantly improve upon current low-redshift
  BAO constraints.  It probes twice the volume of the BOSS LOWZ
  sample, and approximately three times the effective volume.  Given
  the DR11 LOWZ performance from 7300 square degrees, we expect this
  bright-time survey to reach a BAO measurement of $R$ at $z_{\rm
    eff}=0.3$ better than 1\%.  Somewhat better precision may be possible with
  improved density-field reconstruction methods that take fuller
  advantage of the high sampling density.  Adding the BGS to the Figure of Merit
  forecast of \S\ref{sec:scienceForecastResults} for the baseline DESI BAO result, we find that a 14,000 deg$^2$ BGS survey increases
  the FoM from 143 to 176, while 20,000 deg$^2$ brings the FoM to 194.
  These notable improvements reflect the advantage of the low-redshift distance
  scale to constrain $w$.  Alternatively, the BGS BAO result would strengthen 
  the ability to cross-compare BAO and ground-based supernova cosmology results.
  \todo{Put in BAO section.}

\item The BGS will measure the amplitude of clustering at low
  redshift, thereby testing for possible modifications of gravity in
  the regime where dark energy is most important.  This can be tested
  directly via the redshift-distortion method, including the novel
  methods of using multiple tracers in order to suppress sample
  variance \cite{2012PhRvD..86j3513H}.  This can also be tested via
  spectroscopic detection of clusters and groups, along with galaxy
  halo-occupation modeling, to measure the amplitude of clustering by
  halo abundances \cite{2013MNRAS.430..725V, 2012ApJ...745...16T}.
  The maps can also be correlated with weak lensing maps (e.g., from
  DES, LSST, Euclid, or CMB-S4) to measure the amplitude of clustering
  \cite{2012PhRvD..86h3504Y,2013MNRAS.432.1544M}. Finally, comparing
  the observed velocity field to the expected velocity field sourced
  from the lensing matter overdensities enables tests of modified
  gravity models of cosmic acceleration \cite{2010Natur.464..256R}.
  We note that getting the best precision out of the limited volume at
  low redshift requires spectroscopy: one needs a 3-D map in order to
  use all of the modes of the density field.
  \todo{Put in RSD section.}

\item The BGS will permit detailed tests of the scale dependence of
  galaxy bias.  Control of bias is important to use large-scale
  structure to infer properties of the primordial perturbations, e.g.,
  the spectral tilt and Gaussianity, and thereby test inflationary
  models.  We also can test density-field reconstruction, used in BAO
  analyses, in much richer detail.  While the DESI Key Project
  includes the opportunity to do similar tests, it is always with
  sparser samples.  At low redshift, we can utilize a much richer and
  denser map of our local volume.  As the galaxies are different from
  those in the Key Project, the bias parameters are not immediately 
  applicable, but these tests allow us to test the bias models
  in more detail.
  \todo{Drop this.}

\item The survey will support the coming decade of supernova
  cosmology.  At $z<0.4$, a spectroscopic redshift is essential, lest
  the uncertainty in the redshift dwarf the intrinsic precision of the
  standard candle.  Over a 10-year period, a typical ($L^*$) galaxy
  has at least a 1\% probability of having a detectable SN Ia.  This
  means that the BGS will contain at least $10^5$ supernova host
  galaxies.  Samples of this size can only be achieved with
  multi-object wide-field surveys, and with DESI there is no need to
  wait to select the host galaxies after the explosion.  At $z<0.2$,
  the BGS will include more than half of all SN Ia host galaxies in
  the survey footprint.  Having a pre-existing redshift will also
  enable better allocation of follow-up resources for rare transients
  from surveys such as LSST.
  \todo{2.6.LSST}

\item The BGS will sharply improve the training of low-redshift
  photometric redshifts from cross-correlation techniques
  \cite{2008ApJ...684...88N, 2013arXiv1303.4722M}.  Here, one uses the
  angular cross-correlation between classes of faint objects of
  unknown redshift with objects of known redshift in order to map out
  the redshift distribution of each class.  The BGS will provide by
  far the largest sample of $z<0.4$ objects for such a method.
  \todo{2.6.LSST}

\item Essentially all astrophysical tests of modified gravity theories
  rely on ``screening'' maps: a map that determines the level of
  enhancement of gravitational forces over the GR prediction
  \cite{2013arXiv1309.5389J}.  Such maps require knowledge of the
  3-dimensional distribution of galaxies. This will be significantly
  enhanced by the BGS relative to what has been feasible with SDSS
  \cite{2013ApJ...779...39J}. The increased area will help because
  some tests use rare galaxies, wherever they occur on the sky, and
  nearly all tests will benefit from 3-D information on smaller
  galaxies than accessible with SDSS.  In particular, the fidelity of
  the mass distribution in the proximity of test galaxies will be
  significantly improved.
  \todo{Consider this for the end of the intro of 2.5.}
\end{enumerate}

The BGS will benefit other upcoming cosmology projects, including DES
and notably the P5-recommended LSST and CMB-S4.  Spectroscopic
redshifts enhance the lensing and cluster science from these projects
and provide crucial host galaxy redshifts for LSST SNe work.  The P5
panel also advocated for novel probes of gravity under its small
projects recommendation, which will be partially covered by BGS.

\subsubsection{Other Extragalactic Science}
\todo{This probably should be dropped; it's not as relevant for CD-2.
If it exists, it needs to be generalized to dark time.}

The BGS will increase the sample of low-redshift galaxies by a factor
of 15 beyond SDSS.  Many of the science topics pursued with SDSS will
see immediate benefit.  Analyses that depend on measurements of
environment or higher-point clustering benefit enormously from the
higher density sampling.  Spectroscopy is essential for mapping out
group-scale environments, which appears to be the mass scale most
responsible for the transition from late-type to early-type galaxies.
There are also a number of diverse science cases that depend on having
a large area 3D map of the very nearby Universe.  The BGS will
significantly expand the depth of this map compared to all existing
surveys.

The increase in sample size is particularly useful for studies of
dwarf galaxies, as these are rare in flux-limited samples; the dim end
of the luminosity function is currently best measured by GAMA data,
and here the increase will be $\sim$ 50 times current data.  The low
number density of these dwarfs, both within the Milky Way and in the
field, has been famously suggested as a signature of deviations from
the cold dark matter cosmology \cite{2011MNRAS.415L..40B,
  2014arXiv1407.4665P}.  However, models of galaxy formation are least
constrained in the low-mass/low-luminosity regime, and here in
particular, significant environmental dependence is observed.
Shedding more light on this mystery will require significantly larger
samples that probe a range of environments; the volume probed by the
BGS would provide a big step forward.

An additional extragalactic science case involves LIGO neutron-star
mergers.  Advanced LIGO expects to see these events to about 200
Mpc distance, redshift 0.05.  However, the positional uncertainty
is large, typically 100 square degrees or more.  In the rapid search
for electromagnetic counterparts, the ability to reject optical
transients from higher redshift galaxies will be valuable.  The
BGS will include a large fraction (90+\%) of the stellar mass of
the galaxy population at $z<0.05$ and hence is very likely to include
the host galaxy (for events in this half of the sky).

It is important to note that while photometric redshifts may isolate
low-redshift galaxies from those at higher redshift, photometric
redshifts give only few-percent precision on the quantity $1+z$, and
are significantly worse for the faintest galaxies which are quite sparse in
current samples.  This means that the error on the redshift is quite a bit
larger for a low-redshift galaxy, which implies large uncertainties on
the distance to it and the resulting inference of size and luminosity.
Hence, a spectroscopic map is particularly important at low redshift.

This spectroscopy will have great legacy value in light of the many
imaging data sets that are arriving this decade: DES/DECam, LSST,
Subaru/HSC, VST, 
Euclid, extended WISE, and eROSITA, among others.  
We note that Euclid
spectroscopy will not yield redshifts for most of these objects, as
they lack strong emission lines in the near-infrared.

\subsubsection{The Milky Way Survey: Near-Field Cosmology from Stellar Spectroscopy}
\todo{This probably stays; make it section 2.6.}

As explained above, the BGS will necessarily have unassignable fibers,
and these can efficiently be placed on stars.  
At 17th magnitude, even
a short (8-10 min) DESI exposure measures an excellent spectrum with
$S/N = 25$ per pixel, which will yield the radial velocity to a few
km/s precision and the metallicity.  We expect the BGS to generate
at least 10 million such spectra.

Spectroscopy of individual stars provides radial velocity, effective
temperature, surface gravity, chemical abundance distribution, and
approximate age.  The assembly history of the Milky Way is encoded in
the spatial distributions, kinematics, and chemical composition of the
various distinct Galactic stellar populations. This information can
test cosmological predictions for how galaxies like the Milky Way form
and evolve on small scales that are difficult or impossible to test
elsewhere in the Universe, and provide a critical test of the
small-scale predictions of the $\Lambda$CDM model.

%%% Combined with an estimate of the parallax distance 
%%% and proper motion from the European Space Agency's {\it GAIA} mission, 
%%% we can place each star within a Galactic population census.
%%% Repeating this process with millions of stars constructs
%%% a richly textured, multi-parameter map of the Milky Way.
%%% The kinematics and chemical abundances of these
%%% populations can be used to infer the coupled evolutionary history
%%% of the hierarchical assembly of the Galaxy’s dark matter halo and
%%% the chemical evolution of the stellar populations hosted by its
%%% progenitor subhaloes.

The European Space Agency {\it GAIA} satellite has been successfully
launched and will provide a catalog of parallaxes, proper motions, and
spectrophotometry for a billion point sources down to $V \sim 20$ over
the whole sky. The satellite's RVS spectrograph will supplement those
data with radial velocities for millions of brighter stars, although
the flux limit is still under investigation due to higher than
expected scattered light.  DESI can substantially enhance the science
return from {\it GAIA} by providing radial velocities and
metallicities for stars much fainter than what the {\it GAIA}
spectrograph can provide.  While other projects are planned for
spectroscopic follow-up of {\it GAIA} stars, DESI's higher multiplex,
wide field of view, and extremely rapid reconfiguration give it a
clear advantage. 

The stellar program will put exceptional new constraints on the
distribution of dark matter in the Milky Way, a vital measurement that
links Galactic science, galaxy formation and cosmology.  The Milky Way
gravitational potential can be probed via the rotation of the Milky
Way beyond 15 kiloparsecs, the motions of newly discovered tidal
streams, and the kinematics of bright stars in the distant stellar
halo.  The uncertainty in the Milky Way mass, density profile, and
internal structure currently are critically important systematics in
the interpretation of direct and indirect dark matter searches, and
the measurements possible with the stellar program will substantially
reduce these uncertainties.

Joint metallicity and velocity distribution functions for stars far
beyond the solar neighborhood will reveal the recent assembly
history of the outer disk and vastly improve our understanding of
the structure and formation of the thick disk. The first-ever deep
spectroscopic survey of halo main-sequence turn-off stars to 30
kiloparsecs can be used to reconstruct the history of the Galaxy
in its first two billion years and its interaction with other
galaxies, shedding new light on enigmatic halo substructures like
the Virgo overdensity and Hercules--Aquila cloud. Moreover, a survey
of millions of stars will have huge potential for the discovery
of kinematically and chemically peculiar stars in as-yet unexplored
regions of the Galaxy.



==> 2_Science/science_brightnoncosmo.tex <==
The DESI instrument enables a wide diversity of science beyond
dark energy and cosmology. This science, while not part of the DOE funded activity (either construction or operation) can be efficiently carried out in
the bright moon phases when the main survey cannot take data, and with
synchronous observations using individual fibers not allocated by the
main survey.  These additional science opportunities are beneficial to
the entire DESI effort by potentially increasing the pool of institutional
partners and engaging a critical mass of researchers at each
institution.  This may lead to improvements in main survey science through
additional tests of data reduction pipelines, calibrations, and other
survey infrastructure and also provides an opportunity to investigate the
astrophysics of the galaxy populations used in the main survey
measurements.

The quantity and quality of data provided by the combination of 
DESI's fiber density, field of view and sensitivity will enable qualitatively new 
kinds of investigations in may sub-fields of astrophysics.  Several of these 
science cases were described in earlier planning documents written by the 
BigBOSS Community Workshop \cite{BBCW2012} and the NOAO BigBOSS 
Community Science Committee \cite{BBCWSC2012}.
%(http://ast.noao.edu/sites/default/files/bigboss-csc-report.pdf). 
Here we focus on one such project as an 
example of the scope and potential for bright time science with the DESI 
instrument.  Our discussion here draws on that earlier work. 

\subsubsection{Galactic Archeology Survey}

%Recent observational efforts to understand the formation and evolution
%of galaxies, as well as other large-scale structures in the Universe
%follow two different, but complementary paths.  One path is to study
%faint galaxies at large redshifts to characterize their early phases
%of evolution.  Another is to survey resolved stars in nearby galaxies
%to reconstruct their star formation and chemical evolution history.
%Most of the stars ever born in the Universe are still shining today,
%thus studying resolved stars provides information about these galaxies
%over cosmic time.  This latter approach can be thought of as near-field
%cosmology.  These different observational paths yield complementary
%data: the former provides large-scale global galactic properties of
%young galaxies at high-redshift, while the latter provides high
%spatial, kinematic, and chemical information of ancient stars in the
%local Universe.

Much information about galactic evolution, for the
specific case of a large, barred spiral, resides in the stars of the
Milky Way.  Encoded in the spatial distributions, kinematics, and
chemistry of the various distinct stellar populations is the assembly
history of the Milky Way.  This information can test cosmological 
predictions for how individual galaxies like the Milky Way form and 
evolve on small scales that are difficult or impossible to test elsewhere in the Universe.  
The process of recreating the assembly history of a galaxy by identifying 
recognizable stellar population remnants has been referred to as Galactic Archeology \cite{fbharaa}.

Spectroscopy of individual stars provides the key parameters such as
radial velocity, effective temperature (T$_{\rm eff}$), surface gravity
(usually parameterized as log g), chemical abundance distribution, and
approximate age.  With an estimate of distance to the star, its
Galactic location is set and this spatial position, along with the
other characteristics derived from the spectra provide the necessary
information to place this star within a Galactic population census.
Repeat this process millions of times, over a broad range of positions
in the Milky Way, and a richly textured, multi-parameter map can be
constructed.   The kinematics and chemical abundances of these
populations can be used to infer the coupled evolutionary history 
of the hierarchical assembly of the Galaxy's dark matter halo and the 
chemical evolution of the stellar populations hosted by its progenitor
subhalos \cite{jb08,cooper,eris}.  

%A comprehensive Galactic population census requires spectroscopic data
%for a large number of stars over a significant fraction of the Galaxy.
%Up to now, the small field of view and little time available for
%Galactic surveys have limited near-field cosmology spectroscopy
%studies to targeted, small regions of interest with only
%a few thousand stars, or surveys of a few thousand square degrees and a
%few hundred thousand objects that achieve only sparse sampling of a
%small fraction of the Galaxy's populations.  
The field of view and
sensitivity of DESI will enable large-area, contiguous, deep
spectroscopic surveys of stars in our Galaxy. This will be  an advance analogous to
the advent of wide-field imaging surveys a decade ago that first
established the existence of substructure in our Galaxy \cite{majewski},\cite{newberg} and M31 \cite{ibata}, \cite{pandas}.

%Specific questions that can be addressed with a DESI Galactic survey include: 

%\begin{itemize}
%\item What is the accretion history of the Milky Way?  What fraction
 % of the Milky Way's halo, disk and bulge were accretion events?

%\item What are the star formation and chemical evolution histories of progenitor 
%systems accreted by the Milky Way? How do those properties correlate with the 
%mass and accretion time of the progenitor systems as inferred by the kinematic 
%and spatial information in the leftover debris from the accretion events? 

%\item What role do cosmological mergers and interactions play in shaping the structure 
%and star formation history of the disk and its evolution via secular processes? 

%\end{itemize}

%\textbf{Example Galactic Archeology Survey Parameters}

%The bright-time survey outlined here is designed to exploit the three strengths
%of DESI on the Mayall telescope: a large aperture allowing
%observations to faint magnitudes, a 3-degree wide field-of-view
%providing the ability to cover large areas on the sky, and a massively
%multiplexed 5000-fiber spectrograph.  The survey is designed to use an
%exposure time of 4x1200 second visits per field.  This is a compromise
%between the desire to cover more area in order to overlap many remnant
%stellar populations, and the desire for greater depth to reach larger
%distances and the largest possible survey volume.  The combined
%limiting magnitude and exposure time are set to reach to
%signal-to-noise (S/N) spectra of 25-30 per resolution element for the
%faintest targets in bright moon conditions.  Based on previous
%spectroscopic surveys (e.g., \cite{seguepaper}, S/N = 25 is required for robust estimates of
%the overall chemical abundance and the abundances of subsets of
%elements important for chemical evolution studies, such as the
%alpha-elements synthesized in the supernovae that end the lives of
%massive, short lived stars.
%
%There are two classes of stellar targets, separated by effective temperature. 
%These three target types have complimentary brightness and surface densities,
%and together create a survey that spans a large fraction of the volume of the Galaxy. 

%Cooler stars on the red giant branch (RGB) with T$_{eff} <$ 5000 K, can be observed as
%faint as $r$=18, which can be as distant as 125 kpc for the brightest stars at the
%tip of the RGB.  There are about 63 such stars per DESI field.  Stars on the RGB are 
%difficult to separate from the larger number of low-mass, nearby main sequence
%stars using photometry alone, but the {\it Gaia} astrometric mission will provide
%proper motion and distance information that should improve the selection
%efficiency. 

%Warmer stars on the main sequence, T$_{eff} >$ 5000 K, can be observed to $r$ = 17
%if S/N 25 is required at 4000 \AA.  An important precursor study is to determine
%whether the red part of the spectrum is sufficient for the chemical abundance
%determinations. That would enable survey observations of targets as faint as $r$=18. 
%These stars can be observed to distances of 5 kpc. There are 3800 of these
%targets per DESI field at Galactic latitudes more than 40$^{\circ}$ from the plane, many more
%at lower latitudes.  Thus this survey can fill all or most of the fibers over a large fraction of the sky,
%though is flexible enough to accommodate other programs.

%For an overlapping field placement that yields 5 unique square degrees
%per field, typical for the SEGUE Milky Way survey, this observing
%strategy would cover between 25 and 35 unique square degrees per
%night, or about 2700 deg$^2$ per year if one quarter of the
%time is available to this bright program. The population substructure
%features known so far can be many tens of degrees long, so a fair
%sample of the Galactic halo requires a patch of order 100 degrees on a
%side, for a survey area of at least 10,000 deg$^2$.  A five-year 
%survey conducted during the bright time that can't be used by the main
%DESI program could cover more than 10,000 deg$^2$ and most 
%of the high Galactic latitude sky visible from the Northern hemisphere.  
%This kind of large area is a unique and important feature of the proposed 
%survey, and one that is enabled by DESI's capabilities.  



==> 2_Science/science_context.tex <==
{\it Bob Nichol}

Discuss other planned spectroscopic redshift surveys here. Also discuss 21 cm surveys in this context.


==> 2_Science/science_non_cosmo.tex <==
The DESI instrument enables a wide diversity of science beyond the
Dark Energy and Cosmology science case.  Within the context of the
DESI project, non-cosmology science can be efficiently carried out
without impact to the main survey.  In a few cases non-cosmology
science will directly enhance main science operations.  For example,
the galaxy redshift survey discussed below will improve spectroscopic
redshifts in the magnitude range (and beyond) of the main survey by
providing ideal redshift templates and characterizing redshift
reliability.  Increasing the breadth of science carried out by the
DESI instrument during non-survey operations will increase the pool of
institutional participants and may indirectly lead to improvements in
main survey science via non-survey work on data reduction pipelines,
calibrations, etc.

Observing modes for non-cosmology science with DESI fall within four
main categories: (1) bright moon phase observations while the main
survey will not be operating, (2) dark/grey moon phase when the main
survey targets are not visible or during the commission phase of the
project before main survey operations begin, (3) synchronous
observations with individual fibers not used by main survey, and
finally (4) archival studies using the DESI main survey data itself.

In the following section, we describe a number of unique non-cosmology
science programs enabled by DESI.  In each section we describe the
science goals, the observational mode in which observations can be
carried out in the context of the DESI project, and the technical
requirements needed to successful carry out the state science goals.
The sections below draw heavily on earlier efforts to describe
non-cosmology science with DESI, in particular documents written by
the BigBOSS Community Workshop (arXiv:1211.0285) and the NOAO BBCSC
committee.



\subsection{Galaxy Evolution Redshift Survey}

Understanding the processes by which galaxies form and evolve has been
the driver of some of the largest and most successful projects in
astronomy (SDSS).  Thanks to decades of effort we have made great
strides in understanding the galaxy population as a whole and how it
has evolved and transformed over time. Many of these tremendous
advances were driven by large spectroscopic surveys covering
substantial swaths of lookback time (e.g. SDSS, DEEP2,
zCOSMOS).   

Despite this progress, we are woefully ignorant of some of the
fundamental elements of galaxy evolution: What is the efficiency with
which gas is converted to stars in galaxies and how does this depend
on a galaxy's properties, e.g. halo mass, environment, assembly and
star-formation and feedback history?  What are the star formation,
accretion, assembly, and chemical enrichment histories of galaxies?
What are the relative roles of mergers and star formation in the
growth of galaxies at different stellar and halo masses?

Despite the plan to acquire spectra of 24 million galaxies, the main
DESI survey does not adequate address the above questions for multiple
reasons: 1) The sample is color selected, which makes it impossible to
study the demographics of the whole galaxy population and restricts
the sample to $0.7< z <1.4$; 2) the spatial sampling is too low to
measure galaxy environments or relate galaxies to halo mass; and 3)
the spectra will be too shallow to measure redshifts for
non-star-forming galaxies at interesting masses.    

One potentially interesting mode for exploring galaxy evolution could
be as part of an extensive commissioning run for the main cosmology
survey. By targeting significantly deeper than the main survey and
doing so for a magnitude limited (as opposed to color-selected)
sample, this program would serve to provide much needed redshift
templates in advance of the main survey and would test many aspects of
redshift completeness, targeting selection, etc.


%\subsubsection{Techinical Requirements and Observing Mode}

\subsection{Studying the Intergalactic Diffuse Medium} 

The majority of baryons in our Universe exist within a diffuse medium
outside of stars and galaxies.  The dominant reservoir is the
intergalactic medium (IGM), which is responsible for the well-known
\lyaf~absorption observed in the spectra of quasi-stellar
objects (QSOs). The IGM is a low-density, photoionized gas, which
covers an enormously dynamic range of structure and physics traced by
diffuse media.  Combined with the interstellar media (ISM) within
galaxies, the scientific significance of the IGM and ISM touches
nearly all astrophysical endeavors. This includes cosmology, galaxy
formation, star-formation, stellar/AGN formation and feedback, and
even fundamental physics (temporal variations in the fundamental
constants; the neutrino mass).  The IGM gas is very rarely detected in
emission and therefore is most commonly probed in absorption in the
light from background sources. Therefore, spectroscopic observations
are required. Furthermore, the majority of line-diagnostics of this
gas have energies of several eV or greater implying rest-wavelengths
in the far-UV.

One of the main survey samples for DESI is spectroscopy of more than a
million z ~ 3 QSOs with the explicit goal of measuring a BAO signal
from cross-correlation analysis of the IGM/\lyaf.  For the
brightest QSO sources ($r < 20$), this should provide a sufficient
spectrum for traditional IGM absorption line analysis.  Given the
enormity of the sample, the DESI main survey will provide a quantum
leap in surveys of the diffuse media compared to previous surveys
(SDSS, BOSS), and will provide a tremendous dataset for work on the
diffuse media over an enormous range of cosmic lookback time, $z = 0.3
− 5$.


%\subsubsection{Techinical Requirements and Observing Mode}

\subsection{Galaxy Satellite System around Milky Way Analogs}

The Milky Way's satellite galaxy population provides vital clues to
both galaxy formation and the nature of dark matter.  However, the
Milky Way satellites constitute a small, and perhaps biased, sample
from which it is difficult to extrapolate generic properties.  Current
models of Cold Dark Matter (CDM) galaxy formation over-predict both
the number of satellite galaxies observed around the Milky Way and
their central mass densities.  While it is possible that CDM
predictions are incorrect, or that better treatments of baryonic
physics will eventually fix some of the discrepancy, it is also
plausible that the Milky Way's satellite population is not
representative of a typical Milky Way-mass galaxy.  Properly assessing
discrepancies with CDM requires determining the ``intrinsic''
distribution of satellites around Milky Way-mass dark matter halo, of
which the Milky Way is a single realization.  Photometrically,
satellite galaxies are extremely difficult to distinguish from the
thousands of higher redshift background galaxies, requiring a
substantial spectroscopic survey.

The SDSS has detected satellites similar to the Magellanic Clouds
around $\sim 200$ Milky Way analogs (Tollerud et al.~2011, Busha et
al.~2011, Liu et al.~2010).  Yet, it is below these luminosities that
the MW's satellite properties diverge from galaxy formation
predictions.  Under the assumption that luminosity correlates with
mass, a typical Milky Way-mass galaxy should host more than 14
satellites down to the luminosity of the Fornax dwarf galaxy ($M_r
=-12$), yet we observe only 4, and the satellites we do observe are a
factor of 4 less massive than expected (e.g., Busha et al.~2010,
Strigari et al.~2010, Boylan-Kolchin et al.~2012).

Low mass nearby galaxies ($-16 < M_r < -11$, $0.005 < z < 0.01$,
$D\sim20-45$\,Mpc) are almost indistinguishable from the far more
numerous background galaxy population via photometry alone.  To
identify nearby low mass galaxies requires a SDSS-like spectroscopic
effort down to significantly fainter magnitudes.  {\em At present,
  there are no spectroscopic surveys that cover the relevant range of
  magnitude and redshift.}  The goal of this project is to
characterize the satellite populations for a small number of Milky Way
analogs and to build a training sample of nearby low mass galaxies to
improve the efficiency of finding satellites this regime.  These data
and methods will be applicable to a wide range of studies on low mass
galaxies.  Furthermore, the full spectroscopic sample can be used to
improve the photometric redshifts of a substantial fraction of the
entire SDSS photometric sample, with applications for a wide range of
cosmological and galaxy formation studies.  The DESI spectrograph is
very well-matched to this problem and can efficiency make a
significant impact in our understanding of galaxy formation at low
masses and the connection of low mass satellites to their dark matter
halos.

%\subsubsection{Techinical Requirements and Observing Mode}

\subsection{Galactic Archeology Survey}

Observational efforts to understand the formation and evolution of
galaxies, as well as other large-scale structures in the Universe have
followed two different, but complementary paths in recent years. One
path is to study faint galaxies at large redshifts to characterize
their early phases of evolution. The subsections above are examples of
this type of approach. Another path is to survey resolved stars in
nearby galaxies to probe their star formation and chemical evolution
over cosmic time; this is called linear-field cosmology. These
different observational approaches yield complementary data;
large-scale global galactic properties of young galaxies at
high-redshift, and high spatial, kinematic, and chemical information
of ancient stars in the local Universe.

The highest information density about galactic evolution, for the
specific case of a large, barred spiral, resides in the stars of the
Milky Way. Encoded in the spatial distributions, kinematics, and
chemistry of the various distinct stellar populations is the assembly
history of the Milky Way, which then provides strong constraints on
the formation and evolution of our Galaxy. The process of recreating
the assembly history of a galaxy by identifying recognizable stellar
population remnants has been referred to as Galactic Archeology.


Spectroscopy of individual stars provides the key parameters such as
radial velocity, effective temperature (T$_eff$), surface gravity
(usually parameterized as log g), chemical abundance distribution, and
approximate age.  With an estimate of distance to the star, its
Galactic location is set and this spatial position, along with the
other characteristics derived from the spectra provide the necessary
information to place this star within a Galactic population census.
Repeat this process millions of times, over a broad range of positions
in the Milky Way, and a richly textured, multi-parameter map can be
constructed from which a detailed history of our Galaxy can be drawn.

Current photometric plus relatively small spectroscopic surveys are
just beginning to provide hints of a rich stellar population
substructure that permeates the Milky Way.  Such currently detected
stellar substructure is just the tip of the iceberg awaiting
substantially larger and deeper surveys.


\subsection{Exploring the Time Domain} 

Time resolved spectroscopy is the next frontier in observational
astrophysics. The SDSS initiated the era of large imaging and
spectroscopic surveys, and several ongoing projects like the Palomar
Transient Factory (PTF) and Pan-STARRS are exploiting the rich
phenomenology of time variability using large imaging cameras, but the
spectroscopic time domain remains relatively unexplored.  Some
examples include reverberation mapping and the feeding habits of
supermassive black holes at the centers of galaxies, the magnetic
activity of stars within our own Milky Way, and the search for binary
companions to these stars, which has a direct impact on their ability
to harbor planets that can support life.


==> 2_Science/science_trades.tex <==
\begin{table}[p]
\begin{center}
\caption{\label{tab:FOMtrades}%
  Figure of Merit results from altering the scope of individual
  target classes and survey area.  In each target class, the number density
  is altered by the listed percentage with no change to the redshift
  distribution.  Note that in the first line, the Figure-of-Merit is
  due to existing data, without DESI.
  We also show a case in which the \lyaf\ quasars are 
  limited to 3 observations instead of 4.
  The sixth column shows the change in the number of required fiber-exposures
  (number of fibers assigned, weighted by exposure time), 
  shown as a percentage of the baseline number.  
  The final column shows the Figure of Merit compared 
  to the baseline case, which has a FoM of 143.
}
\begin{tabular}{ccccccrr}
LRG & ELG & LyaF & QSO & Area & \% Fibers & FoM & \% FoM \\
\hline
\input{FoMtrades.tex}
\hline
\end{tabular}
\end{center}
\end{table}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.6\textwidth]{plots/dFoMdexp.pdf}
\end{center}
\caption{\label{fig:dFOMdN}%
The derivative of the BAO Figure of Merit with respect to number of 
exposures (number of fibers times exposure per fiber) required 
for each target class in each redshift bin.
This shows that it is preferable to spend fibers on higher redshift
targets, particularly \lyaf\ quasars.  This is because
the quality of the map at $z<1.1$ is so high as to saturate the 
recovery of the BAO information.  However, it is important to note
that the low values at $z<1.1$ are also because there are multiple
good measurements of the density field; removing one target class
therefore does not substantially remove the BAO information.
The FoM gives no credit to this redundancy, but we see it as an
important systematic check.
%%% i.e., this is weighted
%%% by the same exposure costs used in Table \ref{tab:FOMtrades}.
\pvm{This figure isn't  quite done -- the LyaF line needs to run out to higher 
z, and I need to put in the z~2 quasars in which you don't measure the forest 
but you can cross-correlate with the forest.}
\pvm{Hoping that future version will show the derivative for varying 
all target classes at one redshift together.}
}
\end{figure}

We next consider how the Figure of Merit varies as we alter the target
densities relative to the survey baseline.  The goal here is to
understand variations in performance as a function of quantities such
as fiber number, system throughput, field of view, etc.  As a path to
this, we first consider the marginal Figure of Merit value per target
as a function of target class.  We will find that the ELG targets are
the least valuable per fiber (of course, there are many ELG fibers, so
overall the ELG class is very important).  This leads to the
conclusion that at least for moderate adjustments in the hardware, the
optimum strategy is to vary the ELG density, keeping the other target
classes at the maximum level that can be realized.  We will therefore
tend to focus here on variations in the ELGs.

We stress that there are several caveats in consideration of such
trade-offs.  First, the Figure of Merit does not measure the full
cosmological reach of the statistical errors. For example, it
downweights the potential opportunities for RSD work or improved
reconstruction at higher sampling density or for improved measurement
of power at $k\ll0.1h$/Mpc available at lower density.  Second,
the Figure of Merit does not reflect the margin that
the survey should retain to guard against systematic errors or
hardware under performance.  

Third and of immediate concern, some of the target classes overlap
in redshift, most notably the LRG, ELG, and QSOs at $0.6<z<1.1$.
This is valuable, as it allows a direct repeated measurement of the
BAO with very different types of galaxies, thereby testing the model
dependence of galaxy bias.  However, this systematic check is given no
value in the Figure of Merit.  In this section, we often vary a
single target class.  This has rather little impact on the Figure
of Merit when other classes are measuring the density field at the
same redshift.

Table \ref{tab:FOMtrades} shows the Figure of Merit when varying each
major target class to be 0\%, 50\%, 100\%, and 150\% of the baseline
level.  In all cases, this is for a 14,000 deg$^2$ survey.  We also
show the levels for varying all categories within a 9,000 deg$^2$
survey.

In these calculations, we have simply scaled the $n(z)$ for each
category.  For the 50\% cases, this is a conservative choice, in that
it assumes that we simply subsample each category.  One might hope
that with careful target selection, one could pick the more effective
50\% of targets.  However, it is not clear that picking the brighter
targets is optimal, as this skews the distribution to lower redshift.
More importantly, the primary focus is on the ELGs, and we currently
have only limited ability from ELG photometric redshifts at $z>1$ by
which we could shape the $n(z)$ of this target class.

Figure \ref{fig:dFOMdN} shows the derivative of the log of the Figure of Merit
as a function of number of fiber-exposures (number of fibers times 
exposure time per fiber) for each target class in thin redshift bins.  
Unlike Table \ref{tab:FOMtrades}, these derivatives are for small
changes.

Studying Figure \ref{fig:dFOMdN} and Table \ref{tab:FOMtrades}, we
draw the following conclusions.  

\begin{itemize}
\item Varying the density of all targets to 50\% and 150\% of baseline
 alters the FoM by 69\% and 120\%; hence, more objects are better, but
  at a sublinear and mildly saturating level.  This is as expected:
  DESI aims to reach the sample variance limit in the lower redshift
  portion of its survey volume.

\item A 14,000 deg$^2$ survey at the lower density does mildly better
  than a 9,000 deg$^2$ survey at higher density.  The 9,000 deg$^2$
  survey is 80\% of the baseline FoM, while doing 14,000 deg$^2$ at 64\%
  of the number densities is 79\%.  However, as shown below, a more
  optimal redistribution of the 14,000 deg$^2$ survey, with 50\% of the ELG fibers and 100\% of the
  others, obtains 92\% of the baseline FoM (91\% if we decrease the 
  exposure time on the \lyaf).  Hence, given the
  opportunity, going to a wider survey is better.  
This is a soft
  optimization that might be affected by other concerns, such as the
  availability of the extra imaging footprint.  Again, this is as
  expected: the survey is reaching $nP>1$ over most of its volume,
  particularly the volume at lower redshift, so one should seek new volume
  when one can.  The 9,000 deg$^2$ survey requirement is therefore the
  conservative choice, written to reduce risk on the availability of
  the target imaging.

\item Higher redshift ($z>1.4$) targets have more value per fiber.
This is to be expected: the map at lower redshift is dominated by
sample variance ($nP>1$) at BAO wavenumbers, so that removing an object only mildly
degrades the map. Trading one fiber at low redshift
for one at high redshift is therefore preferred.  Of course, one doesn't
know the redshift of a target before the observation, so this optimization
is sharply constrained by how well target selection can separate
different redshifts.

\item Given that the fiber budget is 65\% ELG, 21\% LRG, 8\%
  \lyaf, and 6\% other QSO, the \lyaf\ fibers
  have the most marginal value, followed by the QSOs, then the LRGs,
  with ELGs being lowest.  This can either be seen from Figure
  \ref{fig:dFOMdN} or from differencing the 150\% and 50\% FoM values
  and dividing by the fiber budget.  One should be careful, however,
  that removing the LRGs decreases the FoM only modestly, because the
  ELGs continue to provide a good measurement the density field at the
  same redshifts, albeit using substantially more fibers.

\end{itemize}

Because of this last result and because the ELGs are 2/3 of the fiber
budget, we regard them as the primary capacitor when varying the
overall number density of the survey.  An additional factor, however,
is that some alternative surveys don't have the same exposure
time in each part of the sky, which limits the spectroscopic depth 
on the \lyaf.

If one decreases the ELG target density (and the number of reserve
fibers) to 50\% of baseline, then the total target density is 66\% of
baseline.  This is similar to the instrument's Key Performance Parameters objective to
%% FIX this reference
threshold variation (60\%) (see \S \ref{sec:surveyplan})
and to the ratio of minimum-to-baseline
survey areas 9000/14,000 (64\%).

Next, we consider some scenarios for altering the survey hardware.

\textit{A) Same field of view, but 36\% fewer fibers (lower fiber
  density)}: 
This corresponds to reducing the number of
spectrographs and increasing the fiber patrol radii, holding the field
of view fixed.  Holding the survey area fixed, one would decrease the
ELG density by a factor of 2.  This yields a FoM of 132, 92\% of
baseline.  
Alternatively, one could decrease the survey area to retain
the ELG density.  This would decrease the area for all surveys, which
is a worse trade (FoM 114, 80\%), even accounting for the modest boost 
in the \lyaf\ exposure times.

\textit{B) 36\% smaller field of view, 36\% fewer fibers (same fiber
  density)}: This corresponds to a case in which one implements fewer
spectrographs but holds the fiber patrol radii fixed, either by
partially filling the baseline field or having a reduced field.  The
minimum 9000 deg$^2$ survey is this case.  One could do 64\% of the area of
the baseline strategy, which yields a FoM of 114, 80\% of baseline.
Alternatively, one could hold the survey area and reduce the ELG
density by a factor of 2 \textit{and} decrease the \lyaf\ exposure time.
This produces a FoM of 130, 91\% of the baseline.  This would be
slightly worse than the previous case (A) because of the drop in the
\lyaf\ to 3 visits.  A concern in the latter case is that we would have
fewer visits to any given point in the survey, which would increase the
challenge of correcting for density-dependent incompleteness from fiber
collisions.

\textit{C) Same field of view and fiber count, 36\% lower pan-chromatic
  instrument throughput}: 
Causes might include poorer throughput,
e.g., because of fiber mis-centering or focal ratio degradation, but
it also would include increased instrument overheads that decrease the
survey speed.  As this increases the time required per square degree of
survey, the analysis is equivalent to the previous case (B), as
one has proportionally less observing resource \textit{and} a limit on
the exposure depth of the \lyaf.

\textit{D) Same field of view and fiber count, 36\% lower throughput in the red}:
This might occur for example because of lower spectral resolution,
which would preferentially affect the ability to work between the
night-sky lines to extract ELG and LRG spectra.  As this would slow
down the bulk of the targets, this analysis is largely equivalent to
case (A), as it would cause us to preferentially lose ELG targets,
without impact on the \lyaf.  A difference is that with more time required
per square degree of survey, we would have fewer passes and hence more 
pressure on correcting for fiber collisions.

On the whole, the trade-offs show that the DESI 14k baseline survey
can withstand some degradation before the statistical errors and
resulting Figure of Merit are severely impacted.  Such margin is
important, as increased survey time to meet the mission need would
incur substantial operations costs that can easily exceed savings
in hardware.  Regarding target selection, protecting the high-redshift
quasars is important, as these have the most impact per fiber.  The
Figure of Merit recommends trading $z<1$ ELGs for higher redshift
ones if possible, although we do want to retain some substantial
overlap of the LRGs and ELGs at $z<1$ as a test of galaxy bias
systematics.


==> 4_Targets/cfht.tex <==
For the 5,000 deg$^2$ of the DESI footprint that is inaccessible to DECam, the most efficient option available before DESI begins operations will be the upgraded MegaCam Red instrument on the Canada France Hawaii Telescope.  
Although MegaCam is currently the most powerful, popular and productive instrument on CFHT, it has poor response in the red.
%Its high $u$-band QE combined with the good UV transmission at its high site remains uniquely powerful. 
%However, in the scientifically ever more important red bands, $i$ and $z$, the current CCDs have poor response and the camera is not competitive. For this reason the CFHT community has recently
By replacing the current detectors with deep depletion, pin-compatible devices 
from e2v, MegaCam Red will boost QE across all bands; simultaneous improvements to the camera controller and filter complement are planned.  
%As well,  there should be some straightforward improvements to the camera controller to decrease 
%read time and a set of modern square high throughput filters should be acquired. 
%The ongoing work to install dome vents to improve image quality and a more efficient approach 
%to queue observing will yield additional gains. For a blue balanced CFHT imaging program 
%the resulting overall speed increase should be nearly a factor of 2 faster than the current MegaCam 
%instrument. With this MegaCam upgrade a red balanced program like the DES would 
%produce a competitive Northern sky survey.
To maximize the scientific impact of the upgraded MegaCam the CFHT community is expected to propose an imaging survey covering up to 9000 deg$^2$ of the northern sky.  Such a survey is likely to be particularly focused on the imaging needs of the {\it Euclid} satellite, for which $ugriz$ photometry is required.  

%
% CFHT u band and image quality give the potential to go beyond the Dark Energy Survey 
%currently beginning at CTIO Blanco telescope with the Dark Energy Camera. 
%Moreover, the upgrade would transform CFHT from being a by-stander, 
%or at best a u band assistant, to a central collaborator as the international community 
%of astronomers and telescopes begins to undertake ambitious all-sky optical-infrared imaging 
%and spectroscopic programs. 
%
%The illustrative surveys require either 1350 hours ($grz$ for DESI, although $ugr$ and other 
%3 filter combinations are options) or 9000 ($ugriz$ for Euclid) hours, providing stand-alone science 
%in proportion to their time and access to powerful external scientific programs with 
%their own resources. Such large surveys would take approximately two to three times 
%more time with the current MegaCam. We note that MegaCam allows the possibility 
%of bright time for $i$ and $z$ band observations. The power of the upgraded MegaCam merits 
%serious consideration for its best use policy, however the value of the upgrade 
%stands on its own considerable merit.
%
%
%\paragraph{A Northern Sky Survey with DESI Overlap}
%
%The DESI collaboration would benefit tremendously from a multi-band CFHT imaging survey if it were available.
%Indeed, a CFHT imaging survey  would provide uniform images with high quality astrometry and 
%photometry which is very important for accurate fiber positioning that determines spectroscopic efficiency.

To attain the {\sl grz} depths of 24/23.6/23 AB mag for DESI over 5,000 deg$^2$ would require roughly 180 nights with MegaCam Red; a survey in $z$ alone would require 86 nights, within the range of previous CFHT Large Programs.   By comparison, imaging for {\it Euclid} (which has overlapping needs) is expected to require $\sim 1000$ nights with MegaCam Red.
For our baseline plan, we assume that CFHT/MegaCam Red will provide our $z$-band imaging, while $g$ and $r$ will come from the Bok telescope ({\it q.v.}~below).  The next-best option for $z$-band imaging would be the Mosaic-1.1 camera on the Mayall telescope. %
%%DESI needs a well-controlled sky sample, but does not need photometric redshifts. 
%%Indeed simple color-color cuts using for example $grz$ band data and the WISE [3.4] micron 
%%filter provide the samples they need with relatively little loss to objects outside their 
%%desired redshift ranges. 
%The required {\sl grz} data is 24/23.6/23 AB mag, 
%which would take $\sim$240 sec per pointing. For split exposures covering their 
%entire 9000 deg$^2$ it would take some 1325 CFHT
%hours, about 15\% of the time to do the foreseen 7500 deg$^2$ Euclid survey. 
%There are other 3 filter combinations, such as {\sl ugr} that would satisfy DESI requirements 
%and boost observing efficiency at the cost of requiring dark times. 
%Also, additional science, such as galactic structure, could justify additional filters, 
%all of which can be addressed in some future observing time proposal. 
%The required time is about 50\% larger than the largest programs currently granted under normal 
%CFHT Large Program rules. 
%The Euclid oriented survey has more bands and deeper images than the DESI oriented survey, 
%which provides additional opportunities for imaging science. 

\subsubsection{The Bok Telescope} 
\label{sec:bok}

Our targeting alternatives analysis found that in the $g$ and $r$ bands, a much smaller telescope, the 90-inch (2.3-m) Bok telescope at Kitt Peak, is roughly half as efficient as CFHT/MegaCam would be (in terms of total observing time required).   Since considerably more time may be available on the Bok,  it is a competitive option in these bands.  The telescope is outfitted with a mosaic of four 4k$\times$4k 
CCDs covering a 1 deg$^2$ field in combination.  A survey of the 5,000 deg$^2$ not targeted by DECam in $g$ and $r$ is estimated to require 180 nights on the Bok, an amount of time whose estimated value is comparable to and could be implemented as a DESI buy-in for Steward Observatory (now being negotiated).



